IMO$^3$: Interactive Multi-Objective Off-Policy Optimization

Most real-world optimization problems have multiple objectives. A system designer needs to find a policy that trades off these objectives to reach a desired operating point. This problem has been studied extensively in the setting of known objective functions. We consider a more practical but challenging setting of unknown objective functions. In industry, this problem is mostly approached with online A/B testing, which is often costly and inefficient. As an alternative, we propose interactive multi-objective off-policy optimization (IMO$^3$). The key idea in our approach is to interact with a system designer using policies evaluated in an off-policy fashion to uncover which policy maximizes her unknown utility function. We theoretically show that IMO$^3$ identifies a near-optimal policy with high probability, depending on the amount of feedback from the designer and training data for off-policy estimation. We demonstrate its effectiveness empirically on multiple multi-objective optimization problems.

==> summary_eqs.tex <==
\begin{algorithm}
\caption{Random $\theta$.}
\label{alg:random_theta}
\begin{flushleft}
\hspace*{\algorithmicindent}\textbf{Input:} Logging policy $\pi_0$, logged data $\mathcal{D}$, \\ 
\hspace*{\algorithmicindent} \qquad\;\; initial preference vector $\theta_0$, budget $T$
\end{flushleft}
\begin{algorithmic}[1]
\For{$t=1,\dots,T$} 
    \State Sample $\theta_t$ from a unit ball
    \State $\pi_t \gets \argmax_{\pi\in\Pi} u_{\theta_t} \big(\hat V(\pi)\big)$ 
    % $\pi_t = \argmax_{\pi\in\Theta} w_{t}^\top \hat V(\pi)$ \Comment{Add any exploration here?}
    \State Present $\hat V(\pi_t)$ to the designer 
    \State Receive feedback $Y_t$ % \sim \mathrm{Ber}\big(\ell(\hat V(\pi)); \theta_*\big)$ 
    % \todon{Here we should not say $Y_t$ is sampled from a Bernoulli distribution, right? Because in real application, $Y_t$ should be the designer's response.} 
    % \State \label{update_w}Update $\theta_{t}$ and $H_t$ to get $\theta_{t+1}$ and $H_{t+1}$ based on all observations of $\hat V(\pi_t)$ and $Y_t$, as defined in \eqref{eq:update theta} and \eqref{eq:update H}
    \EndFor
\State Estimate $\tilde\theta$ based on all observations of $\hat V(\pi_t)$ and $Y_t$
\State Return $\tilde\pi_* \gets \argmax_{\pi\in\Pi} u_{\tilde\theta} \big(\hat V(\pi)\big)$ 
\end{algorithmic}
\end{algorithm}
